Channel Customization for Joint Tx-RISs-Rx Design in Hybrid mmWave Systems

In strong line-of-sight millimeter-wave (mmWave) wireless systems, the rank-deficient channel severely hampers spatial multiplexing. To address this inherent deficiency, multiple reconfigurable-intelligent-surfaces (RISs) are introduced in this study to customize the wireless channel. Utilizing the RIS to reshape electromagnetic waves, we theoretically show that a favorable channel with an arbitrary tunable rank and a minimized truncated condition number can be established by elaborately designing the placement and reflection matrix of RISs. Different from existing works on multi-RISs, the number of elements needed for each RIS to combat the path loss and the limited phase control is also considered. On the basis of the proposed channel customization, a joint transmitter-RISs-receiver (Tx-RISs-Rx) design under a hybrid mmWave system is investigated to maximize the spectral efficiency. Using the proposed scheme, the optimal singular value decomposition-based hybrid beamforming at the Tx and Rx can be obtained without matrix decomposition for the digital and analog beamforming. The bottoms of the sub-channel mode in the water-filling algorithm, which are conventionally uncontrollable, are proven to be independently adjustable by RISs. Moreover, the transmit power required for realizing multi-stream transmission is derived. Numerical results are presented to verify our theoretical analysis and exhibit substantial gains over systems without RISs.

==> macro.TeX <==


    %\newcommand{\tr}{\mbox{trace}}
    \def\bm#1{\boldsymbol{#1}}
    \def\ang#1{\mbox{$\langle #1 \rangle$}}
    \def\aang#1{\mbox{$\langle\!\langle #1 \rangle\!\rangle$}}

    \def\mnorm#1{\mbox{$\left|\!\left|\!\left|\, #1 \,\right|\!\right|\!\right|$}}



    \def\Complex{{\rm\rule[.23ex]{.03em}{1.1ex}\kern-.3em{C}}}
    \def\bms#1{\mbox{\boldmath $\scriptstyle #1$}}
    \def\eqover#1{\mbox{$\buildrel #1 \over =$}}
    \def\leqover#1{\mbox{$\buildrel #1 \over \leq$}}
    \def\Imag#1{\mbox{${\Im}\left\{ #1 \right\}$}}
    \def\dist{\mbox{${\sf dist}(z, {\mathbb R}^+)$}}
    \def\largeN{\mbox{${\cal N}$}}

    \newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}}
    \newcommand{\bea}{\begin{eqnarray}} \newcommand{\eea}{\end{eqnarray}}
    \newcommand{\benum}{\begin{enumerate}} \newcommand{\eenum}{\end{enumerate}}
    \def\proof{\noindent\hspace{2em}{\itshape Proof: }}
    \def\aproof{\noindent\hspace{2em}{\itshape Alternative Proof: }}
    \def\endproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}
    \def\endaproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}

  %\newtheorem{theorem}{Theorem}
  %\newtheorem{conjecture}{Conjecture}
  %\newtheorem{definition}{Definition}
  %\newtheorem{example}{Example}
  %\newtheorem{lemma}{Lemma}
  %\newtheorem{proposition}{Proposition}
  %\newtheorem{claim}{Claim}

  \def \veclen {0.8}
  \def \uppos{1.2}
  \def \lowpos{-1.5}
  \def \recwid{0.6}
  \def \rechig{0.4}
  \def \crad{0.25}

  \def \Fwid{0.8}

  \newcommand{\tbox}[1]{%

     \bsegment
      \realmult {\rechig}{0.5} \ta
      \realmult {\recwid}{0.5} \tb
       \lvec (0 \ta)    \lvec ({\recwid} \ta)
       \lvec ({\recwid} -\ta) \lvec (0 -\ta)\lvec (0 0)
       \textref h:C v:C \htext ({\tb} 0){#1}
       \savepos ({\recwid} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}

  \newcommand{\tcir}[1]{%
     \bsegment
     \realmult {\crad}{2} \ta
       \move({\crad} 0)
       \lcir r:{\crad}
       \textref h:C v:C \htext ({\crad} 0) {#1}
       \savepos ({\ta} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}


  \newcommand{\tupnoisec}[1]{%
     \bsegment
     \realadd{\crad}{0.35}\arrowlen
     \realadd{\arrowlen}{0.08}\txtpos
     \rmove({-\crad} \arrowlen) \avec({-\crad} \crad)
     \textref h:C v:C \htext ({-\crad} \txtpos){#1}
     \esegment}

    %%%%%% DEFINITION %%%%%%%%%%%%%%
    \newcommand{\qa}{{\bf a}}
    \newcommand{\qb}{{\bf b}}
    \newcommand{\qc}{{\bf c}}
    \newcommand{\qd}{{\bf d}}
    \newcommand{\qe}{{\bf e}}
    \newcommand{\qf}{{\bf f}}
    \newcommand{\qg}{{\bf g}}
    \newcommand{\qh}{{\bf h}}
    \newcommand{\qi}{{\bf i}}
    \newcommand{\qj}{{\bf j}}
    \newcommand{\qk}{{\bf k}}
    \newcommand{\ql}{{\bf l}}
    \newcommand{\qm}{{\bf m}}
    \newcommand{\qn}{{\bf n}}
    \newcommand{\qo}{{\bf o}}
    \newcommand{\qp}{{\bf p}}
    \newcommand{\qq}{{\bf q}}
    \newcommand{\qr}{{\bf r}}
    \newcommand{\qs}{{\bf s}}
    \newcommand{\qt}{{\bf t}}
    \newcommand{\qu}{{\bf u}}
    \newcommand{\qv}{{\bf v}}
    \newcommand{\qw}{{\bf w}}
    \newcommand{\qx}{{\bf x}}
    \newcommand{\qy}{{\bf y}}
    \newcommand{\qz}{{\bf z}}

    \newcommand{\qA}{{\bf A}}
    \newcommand{\qB}{{\bf B}}
    \newcommand{\qC}{{\bf C}}
    \newcommand{\qD}{{\bf D}}
    \newcommand{\qE}{{\bf E}}
    \newcommand{\qF}{{\bf F}}
    \newcommand{\qG}{{\bf G}}
    \newcommand{\qH}{{\bf H}}
    \newcommand{\qI}{{\bf I}}
    \newcommand{\qJ}{{\bf J}}
    \newcommand{\qK}{{\bf K}}
    \newcommand{\qL}{{\bf L}}
    \newcommand{\qM}{{\bf M}}
    \newcommand{\qN}{{\bf N}}
    \newcommand{\qO}{{\bf O}}
    \newcommand{\qP}{{\bf P}}
    \newcommand{\qQ}{{\bf Q}}
    \newcommand{\qR}{{\bf R}}
    \newcommand{\qS}{{\bf S}}
    \newcommand{\qT}{{\bf T}}
    \newcommand{\qU}{{\bf U}}
    \newcommand{\qV}{{\bf V}}
    \newcommand{\qW}{{\bf W}}
    \newcommand{\qX}{{\bf X}}
    \newcommand{\qY}{{\bf Y}}
    \newcommand{\qZ}{{\bf Z}}
    \newcommand{\qzero}{{\bf 0}}
    \newcommand{\qone}{{\bf 1}}
    \newcommand{\qdh}{\triangle\qh}
    \newcommand{\qhh}{\hat\qh}
    \newcommand{\qdH}{\triangle\qH}
    \newcommand{\qhH}{\hat\qH}
    \newcommand{\qdF}{\triangle\qF}
    \newcommand{\qhF}{\hat\qF}
    \newcommand{\qbh}{\bar\qh}
    \newcommand{\qbn}{\bar\qn}

    \newcommand{\qwbE}{\overline{\bf E}}
    \newcommand{\qwbF}{\overline{\bf F}}
    \newcommand{\qwbT}{\overline{\bf T}}
    \newcommand{\qwbR}{\overline{\bf R}}

    \newcommand{\qDelta}{{\boldsymbol \Delta}}
    \newcommand{\qPsi}{{\boldsymbol \Psi}}
    \newcommand{\qPhi}{{\boldsymbol \Phi}}
    \newcommand{\qXi}{{\boldsymbol \Xi}}
    \newcommand{\qTheta}{{\boldsymbol \Theta}}
    \newcommand{\qLambda}{{\boldsymbol \Lambda}}
    \newcommand{\qSigma}{{\boldsymbol \Sigma}}
    \newcommand{\qGamma}{{\boldsymbol \Gamma}}
    \newcommand{\qUpsilon}{{\boldsymbol \Upsilon}}
    \newcommand{\qOmega}{{\boldsymbol \Omega}}
    \newcommand{\qPi}{{\boldsymbol \Pi}}

    \newcommand{\qalpha}{{\boldsymbol \alpha}}
    \newcommand{\qbeta}{{\boldsymbol \beta}}
    \newcommand{\qdelta}{{\boldsymbol \delta}}
    \newcommand{\qlambda}{{\boldsymbol \lambda}}
    \newcommand{\qgamma}{{\boldsymbol \gamma}}
    \newcommand{\qepsilon}{{\boldsymbol \epsilon}}
    \newcommand{\qeta}{{\boldsymbol \eta}}
    \newcommand{\qnu}{{\boldsymbol \nu}}
    \newcommand{\qmu}{{\boldsymbol \mu}}
    \newcommand{\qkappa}{{\boldsymbol \kappa}}
    \newcommand{\qtau}{{\boldsymbol \tau}}
    \newcommand{\qxi}{{\boldsymbol \xi}}
    \newcommand{\qzeta}{{\boldsymbol \zeta}}
    \newcommand{\qvarepsilon}{{\boldsymbol \varepsilon}}
    \newcommand{\qomega}{{\boldsymbol \omega}}

    \newcommand{\tH}{{\tilde{H}}}
    \newcommand{\tQ}{{\tilde{Q}}}
    \newcommand{\talpha}{{\tilde{\alpha}}}
    \newcommand{\ttau}{{\tilde{\tau}}}

    \newcommand{\tb}{{\tilde{b}}}
    \newcommand{\tc}{{\tilde{c}}}
    \newcommand{\te}{{\tilde{e}}}
    \newcommand{\tm}{{\tilde{m}}}
    \newcommand{\tq}{{\tilde{q}}}
    \newcommand{\tv}{{\tilde{v}}}
    \newcommand{\trho}{{\tilde{\rho}}}
    \newcommand{\tvarepsilon}{{\tilde{\varepsilon}}}

    \newcommand{\tqh}{{\tilde{\qh}}}
    \newcommand{\tqv}{{\tilde{\qv}}}
    \newcommand{\tqH}{{\tilde{\qH}}}
    \newcommand{\tqU}{{\tilde{\qU}}}
    \newcommand{\tqV}{{\tilde{\qV}}}
    \newcommand{\tqD}{{\tilde{\qD}}}
    \newcommand{\tqQ}{{\tilde{\qQ}}}
    \newcommand{\tchi}{{\tilde{\chi}}}
    \newcommand{\tqTheta}{{\tilde{\qTheta}}}
    \newcommand{\tqDelta}{{\tilde{\qDelta}}}
    \newcommand{\tqPsi}{{\tilde{\qPsi}}}
    \newcommand{\tqPhi}{{\tilde{\qPhi}}}
    \newcommand{\tcalqS}{{\tilde{\calqS}}}
    \newcommand{\tqXi}{{\tilde{\qXi}}}

    \newcommand{\tqLambda}{{\tilde{\qLambda}}}

    \newcommand{\hQ}{{\hat{Q}}}

    %\newcommand{\hm}{{\hat{m}}}
    \newcommand{\hchi}{{\hat{\chi}}}

    \newcommand{\hr}{{\hat{r}}}
    \newcommand{\hs}{{\hat{s}}}
    \newcommand{\hq}{{\hat{q}}}
    \newcommand{\hp}{{\hat{p}}}
    \newcommand{\bp}{{\bar{p}}}
    \newcommand{\bv}{{\bar{v}}}
    \newcommand{\bH}{{\bar{H}}}
    \newcommand{\bqH}{{\bar{\qH}}}

    \newcommand{\whqX}{{\widehat{\qX}}}
    \newcommand{\whqZ}{{\widehat{\qZ}}}
    \newcommand{\whqH}{{\widehat{\qH}}}
    \newcommand{\whX}{{\widehat{X}}}
    \newcommand{\whH}{{\widehat{H}}}
    \newcommand{\whZ}{{\widehat{Z}}}

    \newcommand{\wtqY}{{\widetilde{\qY}}}
    \newcommand{\wtY}{{\widetilde{Y}}}
    \newcommand{\wty}{{\widetilde{y}}}


    \newcommand{\uqB}{{\underline{\qB}}}
    \newcommand{\uH}{{\underline{H}}}
    \newcommand{\utH}{{\underline{\tH}}}
    \newcommand{\ubH}{{\underline{\bH}}}
    \newcommand{\uR}{{\underline{R}}}
    \newcommand{\uT}{{\underline{T}}}
    \newcommand{\uqH}{{\underline{\qH}}}
    \newcommand{\uqR}{{\underline{\qR}}}
    \newcommand{\uqT}{{\underline{\qT}}}
    \newcommand{\ubqH}{{\underline{\bqH}}}
    \newcommand{\utqH}{{\underline{\tqH}}}
    \newcommand{\ucalqX}{{\underline{\calqX}}}
    \newcommand{\uqX}{{\underline{\qX}}}

    \newcommand{\bbB}{{\mathbb B}}
    \newcommand{\bbE}{{\mathbb E}}
    \newcommand{\bbN}{{\mathbb N}}
    \newcommand{\bbR}{{\mathbb R}}
    \newcommand{\bbC}{{\mathbb C}}
    \newcommand{\bbS}{{\mathbb S}}
    \newcommand{\bbU}{{\mathbb U}}
    \newcommand{\bbQ}{{\mathbb Q}}

    \newcommand{\calA}{{\mathcal A}}
    \newcommand{\calB}{{\mathcal B}}
    \newcommand{\calC}{{\mathcal C}}
    \newcommand{\calD}{{\mathcal D}}
    \newcommand{\calE}{{\mathcal E}}
    \newcommand{\calF}{{\mathcal F}}
    \newcommand{\calG}{{\mathcal G}}
    \newcommand{\calI}{{\mathcal I}}
    \newcommand{\calK}{{\mathcal K}}
    \newcommand{\calL}{{\mathcal L}}
    \newcommand{\calM}{{\mathcal M}}
    \newcommand{\calN}{{\mathcal N}}
    \newcommand{\calS}{{\mathcal S}}
    \newcommand{\calT}{{\mathcal T}}
    \newcommand{\calO}{{\mathcal O}}
    \newcommand{\calQ}{{\mathcal Q}}
    \newcommand{\calR}{{\mathcal R}}
    \newcommand{\calV}{{\mathcal V}}
    \newcommand{\calX}{{\mathcal X}}

    \newcommand{\calqA}{\boldsymbol{\cal A}}
    \newcommand{\calqB}{\boldsymbol{\cal B}}
    \newcommand{\calqH}{\boldsymbol{\cal H}}
    \newcommand{\calqX}{\boldsymbol{\cal X}}
    \newcommand{\calqQ}{\boldsymbol{\cal Q}}
    \newcommand{\calqS}{\boldsymbol{\cal S}}
    \newcommand{\calqZ}{\boldsymbol{\cal Z}}



    \newcommand{\dom}{{\sf dom}}
    \newcommand{\epi}{{\sf epi}}
    \newcommand{\diag}{{\sf diag}}
    \newcommand{\supp}{{\sf supp}}
    \newcommand{\tr}{{\sf tr}}
    \newcommand{\Ex}{{\sf E}}
    \newcommand{\rank}{{\sf rank}}
    \newcommand{\Varx}{{\sf Var}}
    \newcommand{\Extr}{\operatornamewithlimits{\sf Extr}}
    \newcommand{\mmse}{{\sf mmse}}
    \newcommand{\mse}{{\sf mse}}
    \newcommand{\vect}{{\sf vec}}
    \newcommand*{\argmin}{\operatornamewithlimits{argmin}\limits}
    \newcommand*{\argmax}{\operatornamewithlimits{argmax}\limits}
    \newcommand{\sfQ}{{\sf Q}}
    \newcommand{\sign}{{\sf sign}}


    \newcommand{\rmd}{{\rm d}}
    \newcommand{\rmD}{{\rm D}}

    \newcommand{\sfa}{{\sf a}}
    \newcommand{\sfb}{{\sf b}}
    \newcommand{\sfc}{{\sf c}}
    \newcommand{\sfd}{{\sf d}}
    \newcommand{\sfe}{{\sf e}}
    \newcommand{\sff}{{\sf f}}
    \newcommand{\sfg}{{\sf g}}
    \newcommand{\sfh}{{\sf h}}
    \newcommand{\sfi}{{\sf i}}
    \newcommand{\sfj}{{\sf j}}
    \newcommand{\sfk}{{\sf k}}
    \newcommand{\sfl}{{\sf l}}
    \newcommand{\sfm}{{\sf m}}
    \newcommand{\sfn}{{\sf n}}
    \newcommand{\sfo}{{\sf o}}
    \newcommand{\sfp}{{\sf p}}
    \newcommand{\sfq}{{\sf q}}
    \newcommand{\sfr}{{\sf r}}
    \newcommand{\sfs}{{\sf s}}
    \newcommand{\sft}{{\sf t}}
    \newcommand{\sfu}{{\sf u}}
    \newcommand{\sfv}{{\sf v}}
    \newcommand{\sfw}{{\sf w}}
    \newcommand{\sfx}{{\sf x}}
    \newcommand{\sfy}{{\sf y}}
    \newcommand{\sfz}{{\sf z}}




    \newcommand{\sfB}{{\sf B}}
    \newcommand{\sfC}{{\sf C}}
    \newcommand{\sfF}{{\sf F}}
    \newcommand{\sfH}{{\sf H}}
    \newcommand{\sfP}{{\sf P}}
    \newcommand{\sfX}{{\sf X}}
    \newcommand{\sfZ}{{\sf Z}}
    \newcommand{\sfqB}{\boldsymbol{\sf B}}
    \newcommand{\sfqH}{\boldsymbol{\sf H}}
    \newcommand{\sfqX}{\boldsymbol{\sf X}}
    \newcommand{\sfqx}{\boldsymbol{\sf x}}
    \newcommand{\sfqh}{\boldsymbol{\sf h}}

    \newcommand{\scP}{\mathscr{P}}
    \newcommand{\scF}{\mathscr{F}}

    \newcommand{\aaa}{\buildrel{\circ}\over{a}}
    \newcommand{\aag}{\buildrel{\circ}\over{g}}
    \newcommand{\aeta}{\buildrel{\circ}\over{\eta}}
    \newcommand{\arho}{\buildrel{\circ}\over{\rho}}
    \newcommand{\aalpha}{\buildrel{\circ}\over{\alpha}}
    \newcommand{\ateta}{\buildrel{\circ}\over{\tilde\eta}}
    \newcommand{\atalpha}{\buildrel{\circ}\over{\tilde\alpha}}
    \newcommand{\atrho}{\buildrel{\circ}\over{\tilde\rho}}


    \newcommand{\bfbl}[1]{\bf \color{blue}#1}
    \newcommand{\bl}[1]{\color{blue}#1}
    \newcommand{\bfrl}[1]{\bf \color{red}#1}
    \newcommand{\rl}[1]{\color{red}#1}
    \newcommand{\bfbrl}[1]{\bf \color{BrickRed}#1}
    \newcommand{\bfbbl}[1]{\bf \color{BlueViolet}#1}




    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

